Quantifier Elimination by Dependency Sequents

We consider the problem of existential quantifier elimination for Boolean formulas in Conjunctive Normal Form (CNF). We present a new method for solving this problem called Derivation of Dependency-Sequents (DDS). A Dependency-sequent (D-sequent) is used to record that a set of quantified variables is redundant under a partial assignment. We introduce a resolution-like operation called join that produces a new D-sequent from two existing D-sequents. We also show that DDS is compositional, i.e. if our input formula is a conjunction of independent formulas, DDS automatically recognizes and exploits this information. We introduce an algorithm based on DDS and present experimental results demonstrating its potential.

==> proofs/old_files/compos_proofs.tex <==
\section*{Proposition of Section~\ref{sec:compos}: Compositionality of \Di}
%
%  Compositionality of DDS
%
\begin{definition}
\label{clause_d_seq}
We will refer to D-sequents derived due to appearance of an empty clause in formula \cof{F}{q} 
(see Subsection~\ref{subsec:atomic_d_sequents}) as \tb{clause D-sequents}.
\end{definition}
%
% Proposition: compositionality of DDS
%
\begin{proposition}[compositionality of DDS]
%\label{prop:compos}
Let $T$ be the search tree built by \Di when solving the QE  problem
$\exists{X}[F_1 \wedge \ldots \wedge F_k]$, $\V{F_i} \cap \V{F_j}= \emptyset$, $i \neq j$. 
Let $X_i = X \cap \V{F_i}$ and $Y_i = \V{F_i} \setminus X$.
The size of  $T$ in the number of nodes
is bounded by $|\V{F}|\cdot(\eta(X_1 \cup Y_1) + \ldots +  \eta(X_k \cup Y_k))$ where 
$\eta(X_i \cup Y_i) =  2 \cdot 3^{|X_i \cup Y_i|} \cdot (|X_i| + 1), i=1,\ldots,k$
no matter how decision branching variables are chosen. 
\end{proposition}
\begin{mmproof}
Denote by $Y$ the set of variables $\V{F} \setminus X$.

We prove this proposition for a slightly modified version of \Di\!\!.  
In the version of \Di shown in Figure~\ref{fig:high_level_descr}, the D-sequents depending on the branching variable are discarded.
The modification is to keep all derived D-sequents. (See the discussion in the first section of the Appendix.) This means that there 
is a set $\Pi$ where all derived D-sequents are stored. We assume that \Di does not derive the same D-sequent twice.
That is if $\Pi$ contains a D-sequent $S$ equal to \Dss{X}{F}{q}{\s{x}}, then the modified \Di declares \s{x} redundant as soon as $S$ 
becomes active  instead of deriving it again.

Let $P$ be a path of $T$ and $n(v)$ be a node of $T$ that is on $P$. Here $v$ is the branching variable selected in the node $n$ by \Di\!\!.
We will call $n(v)$ a \tb{BCP node}, if  the variable $v$
was selected due to its presence in a unit clause of \cof{F}{q}. We will call $P$ an \tb{essential path}, if for every BCP node $n(v)$
lying on $P$ (if any) the latter corresponds to the \ti{right branch} of $n$. That is the variable $v$  is currently assigned
the value \ti{satisfying} the unit clause $C$ of \cof{F}{q} due to which $v$ was picked. Recall that the first value assigned to $v$ by \Di 
falsifies $C$.


Let $d$ denote the total number of nodes lying on essential paths.
Notice that the number of all nodes of $T$ is bounded by $2\cdot d$. The reason is that
a non-essential path   contains a BCP node $n(v)$ where $v$ is assigned the value falsifying the unit clause due to which $v$ was
selected.  So  the last node of this path is the left child of node $n(v)$.
 Thus the number of nodes lying only on non-essential paths is bounded by the
number of BCP nodes of $T$. Since every BCP node lies on an essential path, the total number of nodes of $T$ is bounded by $2\cdot\!d$.


Denote by \Sub{N}{ess\_paths} the total number of essential paths of $T$. Denote by \Sub{N}{res\_cl} the total number
of resolvent clauses generated by \Di\!\!. Denote  by  \Sub{N}{D\_seqs} the total number of D-sequents generated by \Di with the exception
of clause D-sequents.

 We do the rest of the proof  in two steps. First we show that 
$\Sub{N}{ess\_paths}~\leq \Sub{N}{res\_cl}~+~\Sub{N}{D\_seqs}$.
Since a path of $T$ cannot contain   more than $|X \cup Y|$ nodes, this means that the total number of nodes of $T$ is
bounded by $2\cdot |X \cup Y| \cdot (\Sub{N}{res\_cl} + \Sub{N}{D\_seqs})$. In the second step, we show that
 $2 \cdot (\Sub{N}{res\_cl} + \Sub{N}{D\_seqs}) \leq \eta(X_1 \cup Y_1) + \ldots +  \eta(X_k \cup Y_k)$ where 
$\eta(X_i \cup Y_i) =  2\cdot 3^{|X_i \cup Y_i|} \cdot (|X_i| + 1), i=1,\ldots,k$.

\vspace{3pt}
\noindent{FIRST STEP:} To prove that $\Sub{N}{ess\_paths}~\leq~\Sub{N}{res\_cl}~+~\Sub{N}{D\_seqs}$ we show that every essential path of $T$
corresponds to a new resolvent clause or a new D-sequent generated by \Di\!\! that is not a clause D-sequent.
Let $P$ be an essential path of $T$. Let $v \in X \cup Y$ be 
the first variable of $P$ picked by \Di for branching.
 The very fact that $v$ was selected 
means that some of the variables of $X$ were not proved redundant  in \prob{X}{F} yet.
Let us assume the contrary, that is \Di is able to finish $P$ without generating a new clause or a new D-sequent that is not a clause D-sequent. 
This only possible if \Di can assign all free non-redundant variables of $X$ without running into a conflict (in which case a new clause is
generated) or producing a new blocked variable  (in which case a new non-clause D-sequent  is generated). 

Let $x \in X$ be the last variable
assigned by \Di on path $P$. 
That is every other variable of $X$ is either assigned or  proved redundant before making an assignment to $x$.
Let \pnt{q} be the set of assignments on path $P$ made by \Di~before reaching  
the  node $n(x)$, and $X'$ be the set of all redundant variables of $X$ in \cof{F}{q}.
Since variables of $Y$ are assigned before  those of $X$, all non-detached  variables of $Y$ are assigned.
Then the current formula, \ie  formula $\cof{F}{q} \setminus \cf{F}{X'}{q}$ has only two kinds of clauses: 
\begin{itemize}
\item clauses depending only on detached variables of $Y$ or
\item unit clauses that depend only on variable $x$.
\end{itemize}
 The two possibilities for the unit clauses depending on $x$ are as follows.
\begin{itemize}
\item $\cof{F}{q} \setminus \cf{F}{X'}{q}$ contains both clauses $x$ and $\overline{x}$. Then, \Di 
generates a new clause. Contradiction.
\item $\cof{F}{q} \setminus \cf{F}{X'}{q}$ does not contain either $x$ or $\overline{x}$ or both. Then $x$ is blocked and
\Di generates a new non-clause D-sequent. Contradiction.
\end{itemize}

\vspace{3pt}
\noindent{SECOND STEP:} Notice that no clause produced by resolution can share variables of two different subformulas $F_i$ and $F_j$.
This means that for every clause $C$ produced by \Di\!\!, $\V{C} \subseteq (X_i \cup Y_i)$ for some $i$. The total number of clauses
depending on variables of $X_i \cup Y_i$ is $3^{|X_i \cup Y_i|}$. So  $\Sub{N}{res\_cl} \leq 3^{|X_1 \cup Y_1|} + \ldots +   3^{|X_k \cup Y_k|}$.

Now we show that $\Sub{N}{D\_seqs} \leq  |X_1|\cdot 3^{|X_1 \cup Y_1|} + \ldots +  |X_k|\cdot 3^{|X_k \cup Y_k|}$  and hence
 $2\cdot(\Sub{N}{res\_cl} + \Sub{N}{D\_seqs}) \leq \eta(X_1 \cup Y_1) + \ldots +  \eta(X_k \cup Y_k)$.
The idea is to prove that every non-clause D-sequent generated by \Di 
is \tb{limited to} \pnt{F_i}, \ie has the form  \Dss{X}{F}{g}{\s{x}}
where $\Va{g} \subseteq X_i \cup Y_i$ and $x \in  X_i$.  The total number of D-sequents limited to $F_i$ is 
equal to $|X_i| \cdot 3^{|X_i \cup Y_i|}$.  (So the total number of D-sequents limited to $F_i$, $i=1,\ldots,k$ is bounded by 
$|X_1|\cdot 3^{|X_1 \cup Y_1|} + \ldots +   |X_k|\cdot 3^{|X_k \cup Y_k|}$.) The factor $|X_i|$ is the number of
variables appearing on the right side of a D-sequent limited to $F_i$.  The factor $3^{|X_i \cup Y_i|}$ 
specifies the total number of all possible  assignments \pnt{g}.
Recall that due to  Proposition~\ref{prop:form_replacement},  D-sequent \Dss{X}{F}{g}{\s{x}} is invariant to adding  
resolvent clauses to $F$. For that reason, we ignore the left side parameter $F$ when counting
the number of D-sequents limited to $F_i$.


Now we prove that every non-clause D-sequent derived by \Di is limited to a formula $F_i$. We carry out this proof by induction.
Our base statement is that D-sequents of an empty set are limited to $F_i$. It is vacuously true.
 Assume that the non-clause  D-sequents   generated so far are limited to $F_i$  and then show that this holds for the next
non-clause D-sequent $S$.
Let $S$ be a D-sequent \Dss{X}{F}{g}{\s{x}} generated 
for a blocked variable $x \in X_i$. Such a D-sequent  is built as described in Lemma~\ref{lemma:d_seq_blocked_var}. Then \pnt{g}
consists of assignments satisfying \s{x}-clauses of $F$ or being the reason for their redundancy.  Since clauses of different subformulas
cannot be resolved with each other, every \s{x}-clause of $F$ can only have variables of $F_i$ where $x \in \V{F_i}$. 
By the induction hypothesis every non-clause D-sequent is limited to some subformula. On the other hand, \Di looks for blocked variables
when \cof{F}{q} has no empty clause. So, at the time $S$ is derived, no variable of \cof{F}{q} can be redundant due to a clause D-sequent.
This means 
that if a variable $x^*$ of an \s{x}-clause of $F$ is redundant due to D-sequent  \Dss{X}{F}{g^*}{\s{x^*}} then $\Va{g^*} \subseteq \V{F_i}$.
So $\Va{g} \subseteq \V{F_i}$. 


Now consider the case when  $S$ is obtained by joining two D-sequents $S'$, $S''$. Let us consider the following three possibilities
\begin{itemize}
\item Neither $S'$ nor $S''$ is a clause D-sequent. Then according to the induction hypothesis they should be 
limited to $F_i$. (They cannot be limited to different subformulas because then they cannot be joined due to absence of a common variable.)
Then due to  Definition~\ref{def:join_rule}, the D-sequent produced by joining $S'$ and $S''$ is also limited to $F_i$.
%
\item Either $S'$ or $S''$ is a clause  D-sequent. Let us assume for the sake of clarity that this is the D-sequent $S'$.
This means that $S'$ has the form \Dss{X}{F}{g}{\s{x}} where \pnt{g} is the minimum set of assignments falsifying a clause $C$ of
$F$ and $x \in X \setminus \Va{g}$.
Since for any resolvent $C$ of $F$, $\V{C} \subseteq  \V{F_i}$, then $\Va{g} \subseteq \V{F_i}$. By the induction hypothesis,
 $S''$ is limited to $F_j$. Since $S'$ and $S''$ have at least one common variable (at which they are joined), $j$ has to be equal to $i$.
So $x \in X_i$. Then joining $S'$ with  $S''$
produces a D-sequent that is also limited to $F_i$.
%
\item Both $S'$ and $S''$ are clause D-sequents. We do not care about this situation because 
 by joining  $S'$ and $S''$ one obtains a clause D-sequent $\square$
\end{itemize}
\end{mmproof}


% LocalWords:  sequents sequent descr


==> proofs/old_files/derivation.tex <==
%
%  D-sequent for a blocked variable
%
\begin{lemma}
\label{lemma:d_seq_blocked_var}
Let \DS~be a compatible set of  D-sequents for an \ecnf formula \prob{X}{F}.
Let there exist  a constructive multi-order \MO~on  \Xr.
Let \pnt{q} be an assignment to variables of \V{F} such that $\ax \subseteq \pnt{q}$ where \ax is the axis of \DS.
Let $v \in X \setminus (\Va{q}~\cup~\Xr)$ be a blocked variable of \cof{F}{q}.
Then D-sequent \Dss{X}{F}{g}{\s{v}} holds where   \pnt{g} is defined as follows.
For every pair of clauses $C',C''$ of $F$ that can be resolved on variable $v$,  \pnt{g} contains either
\begin{itemize}
% item
\item an assignment satisfying $C'$ or $C''$ or 
\item all the assignments of \pnt{r} such that 
  \begin{itemize}
    \item a D-sequent \Dss{X}{F}{r}{\s{w}} is in \DS~ and 
     \item $C'$ or $C''$ contains variable $w$
   \end{itemize}
\end{itemize}
\end{lemma}
%
% Proof
%
\begin{mmproof}
Denote by $\Psi$ the subset of \DS~comprising of all  D-sequents $(\prob{X}{F},F)\!\!\rightarrow\!\!\s{w}$
such that $w$ is in a \s{v}-clause of $F$
and $\pnt{r} \subseteq \pnt{g}$. From Lemma~\ref{lemma:mergeable_set_multi_order}
 it follows that D-sequent holds \Dss{X}{F}{\axx{\Psi}}{X^{\Psi}}. Notice that variable $w$ is blocked in the formula
$\cof{F}{g} \setminus (\cof{F}{g})^{X^{\Psi}}$. Then  Proposition~\ref{prop:bl_var_red} entails that $w$ is redundant
in $\cof{F}{g} \setminus (\cof{F}{g})^{X^{\Psi}}$. Since, by construction, $\pnt{g} \subseteq \axx{\Psi}$, then Lemma~\ref{lemma:holds_in_subspace}
implies that D-sequent \Dss{X}{F}{\pnt{g}}{X^{\Psi}} holds.
Then from Proposition~\ref{prop:rem_bpts_increm} it follows
that the D-sequent \Dss{X}{F}{\pnt{g}}{X^{\Psi} \cup \s{w}} holds. Finally, Lemma~\ref{lemma:subset} implies that
 \Dss{X}{F}{\pnt{g}}{\s{w}} holds too.
\end{mmproof}
%
% Remark
%
\begin{remark}
\label{rem:d_seq_blocked_var}
In the proof of Lemma~\ref{lemma:d_seq_blocked_var}, we established the correctness of    D-sequent \Dss{X}{F \setminus F^{{X}^{\Psi}}}{g}{\s{w}} 
where $\Psi$ is the set of  D-sequents \Dss{X}{F}{r}{\s{w}} of \DS~such that $\pnt{r} \subseteq \pnt{g}$. Note that 
any D-sequent \Dss{X}{F \setminus F^Z}{g}{\s{w}} where $\Psi \subseteq Z \subseteq \DS$ holds too. The reason
is that $w$ remains blocked as long as  the clauses containing variables of $X^{\Psi}$ are removed from \cof{F}{g} $\square$
\end{remark}



==> proofs/old_files/first_part_correctness.tex <==

%
% Definition: single D-sequent
%
\begin{definition}
Let \prob{X}{F} be an \ecnf formula, \pnt{q} be an assignment to \V{F} and $Z \subseteq (X \setminus \Va{q})$.
We will call D-sequent \Dss{X}{F}{q}{W}{Z} \tb{single-variable} if $|Z|$=1. ???
\end{definition}
%
% Definition: compatible assignments, union of assignments
%
\begin{definition}
Let \pnt{q'} and \pnt{q''} be assignments to variables of a CNF formula $F$.
We will call these assignments \tb{compatible} if no
variable of $\Va{q'} \cap \Va{q''}$ has different values in \pnt{q'} and \pnt{q''}.
Let \pnt{q'} and \pnt{q''} be compatible.  We will call the assignment consisting of all assignments of  \pnt{q'} and \pnt{q''}
 the \tb{union} of \pnt{q'} and \pnt{q''}.
\end{definition}
%
%  Definition: compatible set of D-sequents
%
\begin{definition}
Let \DS~ be a set of single-variable D-sequents for an \ecnf~~for-mula \prob{X}{F}.
We will say that \DS~is \tb{compatible} if for any pair of  D-sequents  \Dss{X}{F}{q'}{\s{v'}}  and \Dss{X}{F}{q''}{\s{v''}} of \DS~
assignments, \pnt{q'} and \pnt{q''} are compatible.
\end{definition}
%
%  Definition: one D-sequent per variable
%
\begin{definition}
Let \DS~ be a compatible set of D-sequents for an \ecnf~~formula \prob{X}{F}.
Denote by {\boldmath \Xr} the set of all variables
of $X$ whose redundancy is stated by D-sequents of \DS. In the following write-up
we assume that {\boldmath $|\Xr| = |\DS|$}. That is for every variable $v$ of \Xr, set \DS~
contains exactly one D-sequent stating the redundancy of $v$. Let $Z$ be a subset of \Xr.
Denote by {\boldmath $\DS(Z)$} the subset of \DS~stating the redundancy of variables of $Z$.
\end{definition}
%
% Definition: axis
%
\begin{definition}
Let \DS~ be a compatible set of D-sequents for an \ecnf~~formula \prob{X}{F}.
 Denote by  \ax
 the assignment that is the union of the assignments of all  \pnt{g}  occurring in   D-sequents  \Dss{X}{F}{g}{\s{v}}
of \DS. We will call \ax the \tb{axis} of \DS.
\end{definition}
%
%  Mergence D-sequent
%
\begin{definition}
\label{def:set_of_d_seqs}
Let \DS~ be a compatible set of  D-sequents for an \ecnf~~formula \prob{X}{F}.
 We will call D-sequent \Dss{X}{F}{\ax}{W^{\DS}}{\Xr}  \tb{the mergence D-sequent} for \DS. ???
We will call set \DS~\tb{mergeable} if the mergence D-sequent of \DS~holds for \prob{X}{F}.
\end{definition}

%
%  Ordered set of D-sequents, constructive variable order
%
\begin{definition}
\label{def:constr_var_order}
Let \DS~be a compatible set of  D-sequents for an \ecnf~~formula \prob{X}{F}.
Let a total order $\prec$ be specified on  \Xr~i.e. for any pair of  variables $v', v'' \in \Xr$, $v' \neq v''$, either
$v' \prec v''$ or $v'' \prec v'$ holds. We will call set \DS~with order $\prec$ \tb{an ordered set of D-sequents}.
We will say that $\prec$ is a \tb{constructive order} if
for every variable $v \in \Xr$, the D-sequents \Dss{X}{F \setminus F^{Z'\cup Z''}}{g}{\s{v}} hold
where $Z' \subseteq Z^{\prec v}$, $Z'' \subseteq Z^{\prec v}$ and
\begin{enumerate}
% item
\item $Z^{\prec v}$ is the set of variables of \Xr~preceding $v$ with respect to order $\prec$.
% item
\item Variable $w$ of $Z^{\prec v}$ is in $Z'$ iff  
$\pnt{s} \subseteq \pnt{g}$ holds where $(\prob{X}{F},\pnt{s})\rightarrow \s{w}$, \Dss{X}{F}{g}{\s{v}}
are the D-sequents of \DS~stating the redundancy of $w,v$.

% item
\item $Z''$ is any subset of variables of  $Z^{\prec v} \setminus Z'$.
\end{enumerate}

\end{definition}
%
% Lemma: D-sequent holds in a subspace
%
\begin{lemma}
\label{lemma:holds_in_subspace}
Let D-sequent \Dss{X}{F}{q}{Z} hold and \pnt{r} be an assignment such that $\pnt{q} \subseteq \pnt{r}$.
Then  D-sequent \Dss{X}{F}{r}{Z} holds too.
\end{lemma}
\begin{mmproof}
Assume the contrary i.e. \Dss{X}{F}{r}{Z} does not hold. Then there is a point \pnt{p} where 
$\pnt{r} \subseteq \pnt{q}$ such that \pnt{p} is  an $X$-removable  $Z'$-boundary point  of \cof{F}{r} 
that is also $X$-removable in $F$. Since $\pnt{q} \subseteq \pnt{r}$,
 the sets of clauses of $F$ falsified by \pnt{p} in \cof{F}{q} and \cof{F}{r} are the same.
So \pnt{p} is a $Z'$-boundary point of \cof{F}{q}. 
Since \pnt{p} is $X$-removable in $F$ it is also  $X$-removable in \cof{F}{q}. (Assume the contrary i.e. 
\pnt{p} is not $X$-removable in \cof{F}{q}. Then an assignment \pnt{s} obtained from \pnt{p} by flipping values
of variables of $X \setminus \Va{q}$ satisfies \cof{F}{q}. Hence \pnt{s} satisfies $F$ as well and so
\pnt{p} is not $X$-removable in $F$.)
Then we have to conclude that the variables of $Z$ are not redundant in \prob{X}{\cof{F}{q}}. Contradiction $\square$
\end{mmproof}

%
% Lemma: Any subset of a set of D-sequents with constructive order is mergeable
%
\begin{lemma}
\label{lemma:mergeable_subsets}
Let \DS~be a compatible set of  D-sequents for an \ecnf~~formula \prob{X}{F}.
Let there exist a constructive order  $\prec$ on \Xr. Then any non-empty subset $\Psi$  of \DS~is a mergeable
set of D-sequents.
\end{lemma}
%
% Proof
%
\begin{mmproof}
Denote by $\Phi$ the set comprising every D-sequent \Dss{X}{F}{g}{\s{v}} of $\Psi$ and  every D-sequent of \DS~specifying
redundancy of variables of every set $Z'$ (see condition 2 of Definition~\ref{def:constr_var_order}). First we prove
that the D-sequent \Dss{X}{F}{\axx{\Phi}}{X^{\Phi}} holds where \axx{\Phi} is the axis for $\Phi$. The fact that this D-sequent holds
implies that  D-sequent \Dss{X}{F}{\axx{\Psi}}{X^{\Psi}} does too. Indeed,
due to condition 2 of 
Definition~\ref{def:constr_var_order}, \axx{\Phi} = \axx{\Psi}. So  \Dss{X}{F}{\axx{\Psi}}{X^{\Phi}} holds.
Besides, since $X^{\Psi} \subseteq X^{\Phi}$, from  Lemma~\ref{lemma:subset} it follows that
the D-sequent \Dss{X}{F}{\axx{\Psi}}{X^{\Psi}} holds and so $\Psi$ is mergeable.

We prove the correctness of the D-sequent \Dss{X}{F}{\axx{\Phi}}{X^{\Phi}} by induction in the size of $\Phi$.

\vspace{5pt}
% Base step
\noindent\tb{Base step.} Assume $|\Phi| = 1$. According to Definition~\ref{def:constr_var_order},
if $\Phi$  contains   only one D-sequent $S$, then the mergence D-sequent is equal to $S$ and so it holds.
%
% Inductive step

\vspace{5pt}
\noindent\tb{Inductive step.} Assume that D-sequent \Dss{X}{F}{\axx{\Phi}}{X^{\Phi}}  holds  if $|\Phi|=k$. 
Let $v$ be the variable following the variables of $X^{\Phi}$ with respect to order $\prec$.
Denote by  $S$ the D-sequent \Dss{X}{F}{g}{\s{v}} of \DS~stating redundancy of $v$.
Since $\prec$ is constructive, then according to Definition~\ref{def:constr_var_order}, a D-sequent \Dss{X}{F \setminus F^Z}{g}{\s{v}}
holds where $Z = X^{\Phi}$.


Let {\boldmath $a^{\Phi \cup \{S\}}$} be the axis for $\Phi \cup \s{S}$. By construction, $\pnt{g} \subseteq ${\boldmath $a^{\Phi \cup \{S\}}$}
and \\  $\axx{\Phi}\subseteq${\boldmath $a^{\Phi \cup \{S\}}$}. So according to Lemma~\ref{lemma:holds_in_subspace}, the D-sequents
(\prob{X}{F},{\boldmath $a^{\Phi \cup \{S\}}$}) $\rightarrow X^{\Phi}$ and 
(\prob{X}{F \setminus F^Z},{\boldmath $a^{\Phi \cup \{S\}}$}) $\rightarrow \s{v}$ hold. 
Finally, taking into account that $Z=X^{\Phi}$, from Proposition~\ref{prop:rem_bpts_increm} it follows that the D-sequent 
(\prob{X}{F},{\boldmath $a^{\Phi \cup \{S\}}$}) $\rightarrow X^{\Phi} \cup \s{v}$ holds. So the set of D-sequents $\Phi \cup \s{S}$ is mergeable.
\end{mmproof}

%
% Definition: a set of D-sequents with a constructive multi-order
%
\begin{definition}
\label{def:constr_multi_order}
Let \DS~ be a compatible set of  D-sequents for an \ecnf~~formula \prob{X}{F}.
Let $H$ denote the set of variables $\V{F} \setminus (\Xr \cup \Va{\ax})$ where \ax is the axis of \DS.
 Let {\boldmath \MO} denote a set of $k$ orders $\s{\prec_1,\ldots,\prec_k}$
specified on  variables of \Xr. We will call \MO~a \tb{constructive multi-order} if for every complete assignment
\pnt{q} to the variables of $H$ there is an order $\prec_i$ of \MO~that is constructive for formula $F$ in subspace \pnt{q}. 
\end{definition}
%
% Lemma: Any subset of D-sequents with constructive multi-order is mergeable
%
\begin{lemma}
\label{lemma:mergeable_set_multi_order}
Let \DS~ be a compatible set of  D-sequents for an \ecnf~~formula \prob{X}{F}.
Let there exist  a constructive multi-order \MO~on  \Xr. Then any non-empty subset $\Psi$ of  \DS~is mergeable.
\end{lemma}
%
%  Proof
%
\begin{mmproof}
Let \pnt{q} be an arbitrary complete  assignment to the variables of $H$. Then there is an order $\prec_i$ of \MO~
that is constructive in subspace \pnt{q}. Using the same arguments as in Lemma~\ref{lemma:mergeable_subsets}, one can show
that $\Psi$ is mergeable  in subspace \pnt{q}. That is the D-sequent \Dss{X}{F}{a}{X^\Psi} holds where \pnt{a}
is the union of \pnt{q} and \axx{\Psi} (the latter being the axis of $\Psi$). By joining all such D-sequents on
variables of $H$, one produces the mergence D-sequent \Dss{X}{F}{\axx{\Psi}}{W^\Psi}{X^\Psi}  $\square$
\end{mmproof}



==> proofs/undo.tex <==
When we say that the variables of a set $Z$ are redundant in \prob{X}{\cof{F}{q}}, we mean that they  are \ti{at least 
virtually redundant} in \prob{X}{\cof{F}{q}} (see Definition~\ref{def:virt_redund} and Remark~\ref{rem:virt_redund}).
-----------------
% 
% Proposition: elimination of boundary points variable by variable
%
\begin{proposition}
%\label{prop:rem_bpts_increm}
Let \prob{X}{F} be a CNF formula and \pnt{q} be an assignment to variables of $F$.
Let the variables of $Z$ be redundant in \prob{X}{\cof{F}{q}} where $Z \subseteq (X \setminus \Va{q})$. Let
a variable  $v$ of $X \setminus (\Va{q} \cup Z)$ be redundant in $\prob{X}{\cof{F}{q} \setminus (\cof{F}{q})^Z}$.
Then the variables of $Z \cup \s{v}$ are redundant in \prob{X}{\cof{F}{q}}.
\end{proposition}
%
% proof
%
\begin{mmproof}
Assume the contrary, that is the variables of $Z \cup \s{v}$ are not redundant. Then from Definition~\ref{def:virt_redund} it follows that
\cof{F}{q} has a $Z'$-boundary point \pnt{p} where $Z' \subseteq Z \cup \s{v}$, $\pnt{q} \subseteq \pnt{p}$ that is 
$X$-removable both in \cof{F}{q} and $F$.
Let us consider the two possible cases:
\begin{itemize}
\item  $v \not\in Z'$ (and so $Z' \subseteq Z$).
Since \pnt{p} is removable both in \cof{F}{q} and $F$, the variables of $Z$ are not redundant in \prob{X}{\cof{F}{q}}. Contradiction.
% item
\item  $v \in Z'$ (and so $Z' \not\subseteq Z$). 
 Then \pnt{p} is a \s{v}-boundary
 point of $\cof{F}{q} \setminus (\cof{F}{q})^Z$.
Indeed,  there has to be a clause  $C$ of \cof{F}{q} 
falsified by \pnt{p} that contains variable $v$.
 Otherwise,  condition c) of the definition of a boundary point is broken because $v$ can be removed from $Z'$ (see Definition~\ref{def:bnd_pnt}) .

\vspace{10pt}
Let $P$ denote the set of all $2^{|X \setminus (\mi{Vars}(\boldsymbol{q}) \cup Z)|}$ 
points obtained from \pnt{p} by flipping 
values of variables of $X \setminus (\Va{q} \cup Z)$.
Let us consider the following two possibilities.
     \begin{itemize}
        \item Every point of $P$ falsifies $\cof{F}{q} \setminus (\cof{F}{q})^Z$. This means that the point \pnt{p}
           is a removable \s{v}-
               boundary point of $\cof{F}{q} \setminus (\cof{F}{q})^Z$. Since $v$ is virtually redundant in $\cof{F}{q} \setminus (\cof{F}{q})^Z$
         then point \pnt{p} cannot be removable in $F$. Contradiction.

\vspace{3pt}
         \item A point \pnt{d} of $P$ satisfies $\cof{F}{q} \setminus (\cof{F}{q})^Z$. Let us consider the following two cases.
            \begin{itemize}
              \item \pnt{d} satisfies \cof{F}{q}. This contradicts the fact that \pnt{p} is
 an $X$-removable $Z'$-boundary point of \cof{F}{q}.
                      (By flipping variables of $X \setminus \Va{q}$
                       one can  obtain a point satisfying \cof{F}{q}.)

              \item \pnt{d} falsifies some clauses of \cof{F}{q}. Since \cof{F}{q} and $\cof{F}{q} \setminus (\cof{F}{q})^Z$
 are different only in $Z$-clauses, \pnt{d} is a $Z''$-boundary point of \cof{F}{q} where $Z'' \subseteq Z$.
 By construction, \pnt{p} and \pnt{d} are different only in values of variables of $X$. So, the fact that 
 \pnt{p} is an $X$-removable $Z'$-boundary point
                            of \cof{F}{q} implies that  \pnt{d} is an $X$-removable  $Z''$-boundary point of \cof{F}{q}.
            Since the variables of $Z$ are virtually redundant in \cof{F}{q},  point \pnt{d} cannot be removable in \prob{X}{F}. 
            This means that \pnt{d} can be turned into an assignment satisfying $F$ by changing only values of variables of $X$.
            Then the same applies to \pnt{p}. Hence
            \pnt{p} is not removable in \prob{X}{F}. Contradiction $\square$
            \end{itemize}
     \end{itemize}
\end{itemize}
\end{mmproof}
------------
%
% Blocked  var
%
\begin{proposition}
%\label{prop:bl_var_red}
Let \prob{X}{F} be an \ecnf{} formula and \pnt{q} be an assignment to \V{F}. Let a variable $v$ of  
 $X \setminus \Va{q}$ be
blocked in \cof{F}{q}. Then $v$ is redundant in \prob{X}{\cof{F}{q}}.
\end{proposition}
%
% Proof
%
\begin{mmproof}
Let us show that $v$ is redundant in \prob{X}{\cof{F}{q}} in terms of Definition~\ref{def:red_vars}
 and hence it is also virtually redundant in \prob{X}{\cof{F}{q}}.
Assume the contrary that is $v$ is not  redundant in \prob{X}{\cof{F}{q}} in terms of Definition~\ref{def:red_vars}. Then there is 
an  $X$-removable \s{v}-boundary point \pnt{p} of \cof{F}{q}. 
Note that the clauses of \cof{F}{q} falsified by \pnt{p} have the same
literal $l(v)$ of variable $v$. Let \pnt{p'} be the point obtained from \pnt{p} by flipping the value of $v$.
According to Lemma~\ref{lemma:twin_bnd_pnts}, one needs to consider only the following two cases.
   \begin{itemize}
     \item \pnt{p'} satisfies \cof{F}{q}. Since \pnt{p'} is obtained from \pnt{p} by changing a variable of $X$,
      \pnt{p} is not  $X$-removable in \cof{F}{q}. Contradiction.
     \item \pnt{p'} falsifies only the clauses of \cof{F}{q} with literal $\overline{l(v)}$. (Point \pnt{p'}
       cannot falsify a clause with literal $l(v)$.) Then there is a pair of clauses $C$ and $C'$ of \cof{F}{q}
 falsified by \pnt{p} and \pnt{p'} respectively
       that have opposite literals only of variable $v$. Hence $v$ is not a blocked variable of \cof{F}{q}.
        Contradiction $\square$
   \end{itemize}
\end{mmproof}
------------
%
% Unsatisfied clause
%
\begin{proposition}
%\label{prop:unsat_clause}
Let \prob{X}{F} be an \ecnf{} formula and \pnt{q} be an assignment to \V{F}. 
Let \cof{F}{q} have an empty clause.
Then the variables of  $X \setminus \Va{q}$ are redundant in \prob{X}{\cof{F}{q}}.
\end{proposition}
%
%
%
\begin{mmproof}
Let us show that the variables of  $X \setminus \Va{q}$ are  redundant in \prob{X}{\cof{F}{q}} in terms of Definition~\ref{def:red_vars}
 and hence they are also virtually redundant in
\prob{X}{\cof{F}{q}}.
According to Proposition~\ref{prop:red_vars}, non-redundancy of variables  of  $X \setminus \Va{q}$ in \prob{X}{\cof{F}{q}} implies
the existence of a $Z$-boundary point where $Z \subseteq (X \setminus \Va{q})$. However, the set of $Z$-boundary points of \cof{F}{q}
is empty. Indeed, on the one hand, \cof{F}{q} contains an empty clause $C$ that is falsified by any point. On the other hand,
according to Definition~\ref{def:bnd_pnt}, if \pnt{p} is a $Z$-boundary point, then $Z$ is a non-empty set that has to contain
at least one variable of every clause falsified by \pnt{p}, in particular, a variable of clause $C$ $\square$
\end{mmproof}
-----------
\begin{proposition}
%\label{prop:form_replacement}
Let \prob{X}{F} be an \ecnf{} formula. Let $H = F \wedge G$ where $F$ implies $G$.
Let \pnt{q} be an assignment to \V{F}.
Then if \Dss{X}{F}{q}{Z} holds, the D-sequent  \Dss{X}{H}{q}{Z} does too.
\end{proposition}
%
% proof
%
\begin{mmproof}
Assume the contrary, \ie \Dss{X}{F}{q}{Z} holds but\Dss{X}{H}{q}{Z}  does not.
According to Definition~\ref{def:d_sequent}, this means  that 
variables of $Z$ are not (virtually) redundant in \cof{H}{q}.
That is, there is an $X$-removable $Z'$-boundary point \pnt{p}  of \cof{H}{q} where $Z' \subseteq Z$
that is also $X$-removable in $F$. 
The fact that the variables of $Z$ are
virtually redundant in \cof{F}{q} means that either
\begin{enumerate}
\item \pnt{p} is not an $X$-removable $Z''$-boundary point of \cof{F}{q}
where $Z'' \subseteq Z$ or
\item  \pnt{p} is an $X$-removable $Z''$-boundary point of \cof{F}{q} but it is not $X$-removable in $F$. 
\end{enumerate}
Let us  consider the first case above. The  three reasons  for \pnt{p} not to be an $X$-removable $Z''$-boundary point of \cof{F}{q}.
%
%
%
\begin{itemize}
\item \pnt{p} satisfies \cof{F}{q}. Then it also satisfies \cof{H}{q} and hence cannot be a boundary point of
 \cof{H}{q}. Contradiction.
\item \pnt{p} is not  a  $Z''$-boundary point of \cof{F}{q} where $Z'' \subseteq Z$. That is \pnt{p} falsifies a
clause $C$ of \cof{F}{q} that does not contain a variable of $Z$.
 Since \cof{H}{q} also contains $C$, 
point \pnt{p} cannot be an $Z'$-boundary point of \cof{H}{q} where $Z' \subseteq Z$. Contradiction.
\item \pnt{p} is a $Z''$-boundary point of \cof{F}{q} where $Z'' \subseteq Z$ but  it is not $X$-removable in \cof{F}{q}. This means that one can 
obtain a point \pnt{s}
 satisfying \cof{F}{q} by flipping values of variables of $X \setminus \Va{q}$ in \pnt{p}.
  Since \pnt{s} also satisfies \cof{H}{q}, one has to conclude that \pnt{p} is not a removable point of \cof{H}{q}. Contradiction.
\end{itemize}
%
Now let us consider the second case above i.e.   \pnt{p} is an $X$-removable $Z''$-boundary point of \cof{F}{q} 
but it is not $X$-removable in $F$. Then one
can  turn \pnt{p} into an assignment \pnt{s} satisfying $F$ by changing only values of variables of $X$.
Since \pnt{s} also satisfies $H$, point \pnt{p} cannot be $X$-removable in $H$. Contradiction $\square$
%
%
\end{mmproof}
-----------
To show the  correctness of join operation (Proposition~\ref{prop:join_rule}),  we need to prove the lemma below.

%
% lemma about subsets of variables redundant modulo local irredundancy
%
\begin{lemma}
\label{lemma:subset}
Let \prob{X}{F} be an \ecnf formula, \pnt{q} be an assignment to variables of \V{F}. Let 
  $Z$ be a subset of variables of $X$ that are  redundant in \prob{X}{\cof{F}{q}}.
Let $Z' \subseteq Z$. Then the variables of $Z'$ are also  redundant in \prob{X}{\cof{F}{q}}.
\end{lemma}
\begin{mmproof}
Assume the contrary, \ie the variables of $Z'$ are not virtually redundant in $F$.
 Then there is a $Z''$-boundary point \pnt{p} that is removable both in  \prob{X}{\cof{F}{q}}
 and \prob{X}{F}  where $\pnt{q} \subseteq \pnt{p}$ and $Z'' \subseteq Z'$.
This means that  \pnt{p} cannot be turned into an assignment satisfying $F$ by changing values of variables of $X$.  Since $Z''$ is also
a subset of $Z$, the existence of point \pnt{p} means that the variables of $Z$ are not  redundant in \prob{X}{\cof{F}{q}} either.
Contradiction $\square$
\end{mmproof}
%
%  The resolution rule of DS-calculus
%
\vspace{10pt}
\begin{proposition}
%\label{prop:join_rule}
Let \prob{X}{F} be an \ecnf{} formula. Let D-sequents $(\prob{X}{F},\pnt{q'})\rightarrow Z$ and  \Dss{X}{F}{q''}{Z}
hold. Let \pnt{q'}, \pnt{q''}
be resolvable on $v \in \V{F}$ and \pnt{q} be the resolvent of \pnt{q'} and \pnt{q''}.
Then, the D-sequent  \Dss{X}{F}{q}{Z}  holds  too.
\end{proposition}
\begin{mmproof}
Assume the contrary, that is the variables of $Z$ are not redundant in \prob{X}{\cof{F}{q}}.
 Then there is a $W$-boundary point \pnt{p} where $W \subseteq Z$ and $\pnt{q} \subseteq \pnt{p}$
 that is removable both in \prob{X}{\cof{F}{q}} and in \prob{X}{F}.
By definition of \pnt{q}, the fact that $\pnt{q} \subseteq \pnt{p}$ implies that $\pnt{q'} \subseteq \pnt{p}$ or $\pnt{q''} \subseteq \pnt{p}$.
Assume, for instance, that $\pnt{q'} \subseteq \pnt{p}$.  From  Lemma~\ref{lemma:subset} it follows,  that the variables
 of  $W$ are redundant in \cof{F}{q'}
as a subset of set $Z$ whose variables are redundant in \prob{X}{\cof{F}{q'}}.
 Since $\pnt{q'} \subseteq \pnt{p}$ and \pnt{p} is a $W$-boundary point of \cof{F}{q}, point \pnt{p}
is also a $W$-boundary point of \cof{F}{q'}. The fact that \pnt{p} is removable in \prob{X}{F}
implies that the variables of $Z$ are not redundant in \prob{X}{\cof{F}{q'}}.  Contradiction $\square$
\end{mmproof}

----------
\input{proofs/first_part_correctness}
\input{proofs/derivation}
------------
\begin{proposition}
%\label{prop:correctness}
\Di is sound and complete.
\end{proposition}
\begin{mmproof}
First, we show that \Di is \ti{complete}. \Di builds a binary search tree and
visits every node of this tree at most three times (when starting the left branch, when backtracking
to start the right branch, when backtracking from the right branch). 
So \Di is complete.

Now we prove that \Di is \ti{sound}.  
\Di terminates in two cases. First, it terminates when an empty clause is
derived, which means that $F$ is unsatisfiable. In this case, the formula $G$ returned by \Di consists
only of an empty clause.
This result is correct because this  clause is built by resolving clauses of $F$ 
and resolution is sound. Second, \Di terminates after building a sequence of D-sequents 
$(\prob{X}{F},\emptyset) \rightarrow \s{x_{i_1}}$, $\ldots$ ,$(\prob{X}{F},\emptyset) \rightarrow \s{x_{i_k}}$
where $x_{i_1},...,x_{i_k}$ are the variables forming $X$. As we show below, the D-sequents derived by \Di
are correct  and a constructive multi-order \MO~holds on the current set of redundant variables 
\Xr~where \DS~is the current set of active D-sequents. Then from Lemma~\ref{lemma:mergeable_set_multi_order}
 it follows that the D-sequent $(\prob{X}{F},\emptyset)\rightarrow X$ holds. This means that the formula
$G$ obtained by dropping the $X$-clauses from the CNF formula $F$ returned by \Di~is equivalent
to \prob{X}{F}.


Now we use induction to prove that the D-sequents derived by \Di are correct and there exists a constructive multi-order
for every set of active D-sequents.
The base statement is that the D-sequents of an empty set are correct and there is a constructive multi-order
on an empty set of D-sequents.  Both these statements are vacuously true.

The induction step  is  to show that if 
\vspace{-5pt}
\begin{itemize}
\item the first $n$ D-sequents derived by \Di~are correct (denote these set of D-sequents as $\Pi$.
\item a constructive multi-order exists on the set \Xr~of variable where $\DS \subseteqq \Pi$ is the current set of active D-sequents
\end{itemize}
\vspace{-5pt}
then 
\vspace{-5pt}
\begin{itemize}
\item next D-sequent $S$  is correct and 
\item a constructive multi-order exists on the set of variable $X^{\DS~\cup~\s{S}}$.
\end{itemize}

 Due to Proposition~\ref{prop:form_replacement}, one can view
the D-sequents of $\Pi \cup \s{S}$ as specified with respect to the current CNF formula $F$.
Let us consider the following alternatives.
\begin{itemize}
\item $S$ is a D-sequent built for  a blocked  variable.
The correctness of $S$ follows from  Lemma~\ref{lemma:d_seq_blocked_var}
and the induction hypothesis (that the D-sequents of $\Pi$ are correct).
The fact that a constructive multi-order exists on the set of variables $X^{\DS~\cup~\s{S}}$ follows from
Remark~\ref{rem:d_seq_blocked_var} and the induction hypothesis.
%
\item $S$ is the D-sequent due to appearance in the current formula a falsified clause $C$. In this case, $S$ is trivially correct.
$S$ remains correct after the set of clauses $F^Z$ is removed from \cof{F}{q} where \pnt{q} is the current set of assignments
and $Z$ is any subset of $X \setminus \Va{q}$. So a constructive multi-order exists on the set of variables  $X^{\DS~\cup~\s{S}}$.
%
\item
 $S$ is obtained by joining two existing D-sequents. The correctness of $S$ follows from 
 Proposition~\ref{prop:join_rule} and the induction hypothesis. The existence of a constructive multi-order 
on the set of variables  $X^{\DS~\cup~\s{S}}$ can be shown as follows. Let $S$ be equal to \Dss{X}{F}{r}{\s{w}}.
Let $S$ be obtained from D-sequents $S_0$ and $S_1$ by joining at variable $v$. 
Let $S_0$ and $S_1$ be equal to \Dss{X}{F}{r_0}{\s{w}} and \Dss{X}{F}{r_1}{\s{w}} respectively. We assume here that \pnt{r_0}
and \pnt{r_1} contain assignments $(v=0)$ and $(v=1)$ respectively.
Assume the contrary i.e. there is no constructive multi-order for $X^{\DS} \cup \s{w}$. This means that a D-sequent $S'$
equal \Dss{X}{F \setminus F^Z}{r}{\s{w}} does not hold where $Z$ is a subset of \Xr. Then  $S'$ does not hold either in 
subspace $\pnt{r} \cup \s{(v=0)}$ or  $\pnt{r} \cup \s{(v=1)}$. Assume for clarity that $S'$ does not hold in the former.
Consider the following two cases.
\begin{itemize}
\item $(v=0)$ is the right branch. Then $S_0$ is currently active and there is no constructive multi-order for the variables of $\Xr$.
This contradicts the induction hypothesis.
\item $(v=0)$ is the left branch. Then there was no constructive multi-order for the variables of $\Xr$ when $S_0$ was active
       in the left branch. This contradicts the induction hypothesis $\square$
\end{itemize}


\end{itemize}
\end{mmproof}
\vspace{5pt}


==> undo.tex <==
\newcommand{\Dss}[4]{\mbox{$(\prob{#1}{#2},\pnt{#3})~\rightarrow #4$}}
\newcommand{\DDs}[4]{\mbox{$(#1,#2,\pnt{#3})~\rightarrow$ \s{#4}}}
----------------
 We introduce
them solely to explain the semantics of \Di\!\!.
----------
Finally, Subsection~\ref{subsec:trivial_cases} describes two cases where proving variable redundancy is trivial.
----------

%
% SUBSECTION
%
\subsection{Decomposing the Problem of Boundary Point Elimination}
\label{subsec:prob_decomp}
----------
%
% Virtual redundancy of variables
%
\begin{definition}
\label{def:virt_redund}
Let \prob{X}{F} be an \ecnf{} formula, \pnt{q} be an assignment to \V{F}, and
$Z \subseteq (X \setminus \Va{q})$.
Variables of  $Z$ are called \tb{virtually redundant} in \prob{X}{\cof{F}{q}} if
$\prob{X}{\cof{F}{q} \setminus (\cof{F}{q})^Z} \equiv \cof{(\prob{X}{F})}{r}$ where $\pnt{r} \subseteq \pnt{q}$ and
$\Va{r} = \Va{q} \setminus X$.
\end{definition}
%
% Remark
\begin{remark}
\label{rem:virt_redund}
Redundancy of variables of $Z$ in \prob{X}{\cof{F}{q}} in terms of Definition~\ref{def:red_vars} is a special case of
virtual redundancy.
To prove variables of $Z$  redundant in \prob{X}{F} in subspace \pnt{q}, it is sufficient to show virtual redundancy of $Z$
in \prob{X}{\cof{F}{q}}. The reason is that one can ignore  $Z$-boundary points that are removable in \prob{X}{\cof{F}{q}} 
and not removable in \prob{X}{F}. We introduce a new notion of redundancy of variables $Z$ in \cof{F}{q} because
the operation of joining D-sequents   preserves only virtual redundancy of $Z$ (Subsection~\ref{subsec:join_d_seqs}).
 In the sequel, when we say that variables of $Z$ are redundant in \prob{X}{\cof{F}{q}} we
mean that they are \tb{at least virtually redundant}.
\end{remark}
------------
\begin{proposition}
\label{prop:rem_bpts_increm}
Let \prob{X}{F} be a CNF formula and \pnt{q} be an assignment to variables of $F$.
Let the variables of $Z$ be redundant in \prob{X}{\cof{F}{q}} where $Z \subseteq (X \setminus \Va{q})$. Let
a variable  $v$ of $X \setminus (\Va{q} \cup Z)$ be redundant in $\prob{X}{\cof{F}{q} \setminus (\cof{F}{q})^Z}$.
Then the variables of $Z \cup \s{v}$ are redundant in \prob{X}{\cof{F}{q}}.
\end{proposition}

Proposition~\ref{prop:rem_bpts_increm} shows that one can make variables of $X \setminus \Va{q}$ redundant \ti{incrementally},
if every \s{v}-clause is removed from \cof{F}{q} as soon as variable $v$ is proved redundant.
-------------
%
%  definition q1 \subseteq q2
%
\begin{definition}
Let \pnt{q_1} and \pnt{q_2} be assignments. The expression
$\pnt{q_1} \subseteq \pnt{q_2}$ denotes the fact that $\Va{q_1} \subseteq \Va{q_2}$ and each variable  of \Va{q_1}
has the same value in \pnt{q_1} and \pnt{q_2}.
% $\pnt{q_1}(v)=\pnt{q_2}(v)$ 
%the  value assignments of \pnt{q_1} are a subset of those of  \pnt{q_2}.
\end{definition}
-------------
%
%  D-sequent
%
\begin{definition}
\label{def:d_sequent}
Let \prob{X}{F} be an \ecnf{} formula. Let \pnt{q} be an assignment to \V{F}
and $Z$ be a subset of $X \setminus \Va{q}$.
A dependency sequent (\textbf{D-sequent})  has the form
$(\prob{X}{F},\pnt{q})\!\rightarrow\!Z$. It states that 
the variables of $Z$ are redundant in  \prob{X}{\cof{F}{q}}.
\end{definition}

% valid D-sequent $(F,X',\pnt{q})~\rightarrow X''$ implies the interdependence of variables of $X',\Va{q},X''$, hence the
% name ``dependency sequent''.

%
% example
%
\begin{example}
Consider an \ecnf{} formula \prob{X}{F} where $F=C_1 \wedge C_2$, 
$C_1=x \vee y_1$ and $C_2=\overline{x} \vee y_2$ and  $X =\{x\}$.
Let \pnt{q}=\s{(y_1=1)}. Then \cof{F}{q} = $C_2$ because $C_1$ is satisfied.
Notice that  $x$ is monotone and so redundant in \cof{F}{q} (Proposition~\ref{prop:bl_var_red}).
Hence, the D-sequent $(\prob{X}{F},\pnt{q}) \rightarrow \s{x}$ holds.
\end{example}
---------
%
%
%\begin{remark}
%\label{rem:join_invariant}
 As we mentioned in Subsection~\ref{subsec:prob_decomp}
the operation join preserves only virtual redundancy of D-sequents.
 The reason is as follows.  ,
A point \pnt{p} that is removable in \cof{F}{q} may not be removable in $F$ (see  Remark~\ref{rem:glob_impl_loc}).
 A similar situation may occur when joining D-sequents
\Dss{X}{F}{q'}{Z} and \Dss{X}{F}{q''}{Z} to produce D-sequent \Dss{X}{F}{q}{Z} (see Definition~\ref{def:join_rule}).
 Let $A(\pnt{q})$ denote the set
of all points obtained by adding to \pnt{q}  assignments to the variables of  $\V{F} \setminus \Va{q}$. 
Then a point \pnt{p} not removable in $A(\pnt{q'}) \cup A(\pnt{q''})$ may 
be removable in  $A(\pnt{q})$ in case $F$ is satisfiable in the former and unsatisfiable in the latter. This may happen if
 $A(\pnt{q}) \subset  A(\pnt{q'}) \cup A(\pnt{q''})$.
%\end{remark}
-------------
%
%  Proposition: safely adding resolvents to F
%
\begin{proposition}
\label{prop:form_replacement}
Let \prob{X}{F} be an \ecnf{} formula. Let $H = F \wedge G$ where $F$ implies $G$.
Let \pnt{q} be an assignment to \V{F}.
Then if \Dss{X}{F}{q}{Z} holds, the D-sequent  \Dss{X}{H}{q}{Z} does too.
\end{proposition}
%

%
% SUBSECTION: Joining D-sequents
%
\subsection{Join Operation for D-sequents}
\label{subsec:join_d_seqs}
In this subsection, we introduce the operation of joining D-sequents.
The join operation
produces a new D-sequent from two D-sequents derived earlier. 
The semantics of this operation in terms of elimination of boundary points is quite simple. 
Let  $A_1$ and $A_2$ be subspaces from which all removable boundary points of $F$ relevant to
redundancy of $Z \subseteq X$ in \prob{X}{F} have been eliminated. The join operation 
produces a new such subspace $A$ where  $A \subseteq A_1 \cup A_2$. 
We start with introducing resolution of  assignments that is similar to
that of clauses.
%
% Resolution of  assignments
%
\begin{definition}
\label{def:res_part_assgns}
Let \pnt{q'} and \pnt{q''} be  assignments in which exactly  one variable $v \in \Va{q'} \cap \Va{q''}$ is assigned different values.
The assignment \pnt{q} consisting of all  the assignments of \pnt{q'} and \pnt{q''} but those to $v$ is called the
 \tb{resolvent} of \pnt{q'},\pnt{q''} on $v$.
Assignments \pnt{q'},\pnt{q''} are called \tb{resolvable}  on $v$.
\end{definition}
%
%  The join rule of DS-calculus
%
\begin{proposition}
\label{prop:join_rule}
Let \prob{X}{F} be an \ecnf{} formula. Let D-sequents $(\prob{X}{F},\pnt{q'})\rightarrow Z$ and  \Dss{X}{F}{q''}{Z}
hold. Let \pnt{q'}, \pnt{q''}
be resolvable on $v \in \V{F}$ and \pnt{q} be the resolvent of \pnt{q'} and \pnt{q''}.
Then, the D-sequent  \Dss{X}{F}{q}{Z}  holds  too.
\end{proposition}
%
% Joining D-sequents
%
\begin{definition}
\label{def:join_rule}
We will say that the D-sequent \Dss{X}{F}{q}{Z} \ of Proposition~\ref{prop:join_rule} is produced 
by \tb{joining D-sequents} \Dss{X}{F}{q'}{Z} and $(\prob{X}{F},\pnt{q''})\rightarrow Z$
at $v$. 
\end{definition}
-----------
In this section, we describe  a QE algorithm called \Di (Derivation of D-Sequents). \Di derives  D-sequents 
 \Dss{X}{F}{r}{\s{x}} stating the redundancy of one variable of $X$.
From now on, we will use a short notation of  D-sequents writing \Dds{r}{\s{x}} instead of \Dss{X}{F}{r}{\s{x}}.  We will assume 
that the parameter  \prob{X}{F} missing in \Dds{r}{\s{x}} is  the \ti{current} \ecnf{} formula (with all resolvent clauses added to $F$ so far).
One can omit \prob{X}{F} from D-sequents because Proposition~\ref{prop:form_replacement} entails that once  a D-sequent $S$
equal to  \Dss{X}{F}{r}{\s{x}}
 is derived by \Di it holds in any future branch \pnt{q} where $S$ is active.  D-sequent $S$ is said to be \tb{active} in branch \pnt{q}
if $\pnt{r} \subseteq \pnt{q}$.
----------
\Di terminates when  for every variable $x$ of $X \setminus \Va{q}$ it derives a D-sequent $\pnt{g} \rightarrow \s{x}$ where $\pnt{g} \subseteq \pnt{q}$.
According to  Proposition~\ref{prop:rem_bpts_increm}, derivation of such D-sequents means  that the D-sequent \Dds{\pnt{q}}{X \setminus \Va{q}} holds.
Proposition~\ref{prop:rem_bpts_increm} is applicable here
because once a variable $x$ of $X \setminus \Va{q}$ is proved redundant in \prob{X}{\cof{F}{q}}, 
every  \s{x}-clause of \cof{F}{q}  is \ti{marked} as redundant. A redundant clause is ignored by \Di until it is unmarked as non-redundant.
So, \Di terminates when the QE problem is solved for $\Phi$ in  subspace \pnt{q}. 
----------
Suppose  no  clause of $F$ is falsified by \pnt{q}. Then for every variable $x$ of $X \setminus \Va{q}$ 
that does not have a D-sequent in \DS~and  is blocked, 
a D-sequent is built  as explained below. This D-sequent is then added to \DS~(line 4). If every variable of $X \setminus \Va{q}$
 has a D-sequent in \DS, then \cof{F}{q} is satisfiable. (If \cof{F}{q} is \ti{unsatisfiable}, 
the variables of $X \setminus \Va{q}$ can be made redundant \ti{only} by adding a clause falsified by \pnt{q}.)
So, the answer \ti{sat} and set \DS~is returned (line 6).

Given a blocked variable $x \in X \setminus \Va{q}$ of \cof{F}{q}, a D-sequent \Dds{g}{\s{x}} is built as follows.
The fact that $x$ is blocked in \cof{F}{q} means that  for any pair of clauses $C'$,$C''$ resolvable on $x$, $C'$ or $C''$  is 
either satisfied by \pnt{q} or redundant (as containing a variable proved redundant in \prob{X}{\cof{F}{q}} earlier). Assume that it is clause $C'$.
 The assignment  \pnt{g} 
is a subset of assignments of \pnt{q} such  that $C'$ is satisfied by \pnt{g} or redundant in \prob{X}{\cof{F}{g}} and
so $x$ is blocked in \cof{F}{g}. If $C'$  is satisfied
by \pnt{q}, then \pnt{g} contains an assignment of \pnt{q} satisfying $C'$. If $C'$ is not satisfied
by \pnt{q} but contains a variable $x^*$ proved redundant earlier, \pnt{g} contains all the assignments of \pnt{g^*}
where \Dds{g^*}{\s{x^*}} is the D-sequent of \DS~stating redundancy of $x^*$.
A proof of correctness of \Dds{g}{\s{x}} is given
in the Appendix (Lemma~\ref{lemma:d_seq_blocked_var}).
--------------
\subsection{Switching from Left to Right Branch}
\label{subsec:left_to_right}
\Di prunes big chunks of the search space by not branching on redundant variables of $X$ or
detached variables of $Y$. One more powerful pruning technique of \Di
discussed in  this subsection  is to reduce  the size of right branches.

Let \Dds{g}{\s{x}} be a  D-sequent of  the set $\DS$~
computed by \Di in the left branch $v=0$ (line 5 of Figure~\ref{fig:high_level_descr}).
 Notice that if \pnt{g} has no assignment $(v\!\!=\!\!0)$, variable $x$ remains redundant
in \prob{X}{\cof{F}{q_1}}  where $\pnt{q_1} = \pnt{q} \cup \s{(v=1)}$. 
This is because  \Dds{g}{\s{x}} is still active in the subspace specified by \pnt{q_1}. 
\Di splits the set $\DS$ into subsets \Sup{\DS}{sym} and \Sup{\DS}{asym} of  D-sequents symmetric and asymmetric
with respect to variable $v$ (line 6). We call a D-sequent \Dds{g}{\s{x}} \ti{symmetric} with respect to $v$,
 if \pnt{g} does not contain an assignment to $v$ and \ti{asymmetric} otherwise.

Denote by \Sup{X}{sym} and \Sup{X}{asym} the variables of $\Sub{X}{red} \setminus \Va{q}$
whose redundancy is stated by D-sequents of  \Sup{\DS}{sym} and \Sup{\DS}{asym} respectively.
Before exploring the right branch (line 9), the variables of \Sup{X}{asym}
become non-redundant again.   Every clause $C$ of \cof{F}{q} with a variable of \Sup{X}{asym} is  unmarked as currently non-redundant unless
%$C$ has a variable of \Sup{X}{sym}.
$\V{C} \cap \Sup{X}{sym} \neq \emptyset$.

Reducing the set of free variables of the right branch to \Sup{X}{asym} allows to prune big parts of the search space.
In particular, if \Sup{X}{asym} is empty there is no need to explore the right branch. In this case, \Di just returns
the results of the left branch (line 7). Pruning the right branch when \Sup{X}{asym} is empty is similar to non-chronological
backtracking well known in SAT-solving~\cite{grasp}.
--------------
\subsection{Branch Merging}
\label{subsec:branch_merging}
Let  $\pnt{q_0}=\pnt{q} \cup \s{(v=0)}$ and $\pnt{q_1}=\pnt{q} \cup \s{(v=1)}$.
The goal of branch merging is to extend the redundancy of all unassigned variables of $X$ proved in \prob{X}{\cof{F}{q_0}} and \prob{X}{\cof{F}{q_1}} 
to formula \prob{X}{\cof{F}{q}}.
If both \cof{F}{q_0} and \cof{F}{q_1} turned out to be unsatisfiable, this
is done as described in lines 11-14 of Figure~\ref{fig:high_level_descr}. 
In this case, the unsatisfied clauses $C_0$ and $C_1$ of \cof{F}{q_0} and \cof{F}{q_1} returned in the left and right branches respectively
are resolved on  $v$.  The resolvent $C$ is added to $F$.  

Since $F$ contains clause $C$ that is falsified
by \pnt{q}, for every variable $x \in X \setminus \Va{q}$ whose D-sequent is not in \DS,
\Di derives an atomic D-sequent  as  described in Subsection~\ref{subsec:atomic_d_sequents}. This D-sequent is then added to \DS.
If, say,  $v \not\in \V{C_1}$, then \ti{resolve\_clauses} (line 11 ) returns $C_1$ itself since $C_1$ is falsified by \pnt{q}
(and so no new clause is added to $F$).

%
\input{m1erge.fig}
%

If at least one branch returns answer \ti{sat}, then \Di calls procedure \ti{merge} described in Figure~\ref{fig:merge}. First,
\ti{merge} takes care of the variables of  \Sup{X}{asym} 
%of  variables whose D-sequents of set \DS~returned in the left branch depended on assignment $v=0$ 
(see Subsection~\ref{subsec:left_to_right}).
Note that redundancy of  variables of \Sup{X}{asym} is already proved in both branches. 
If a D-sequent of a variable from \Sup{X}{asym} returned in the \ti{right} branch is asymmetric in $v$,
then \ti{join\_D\_seqs} (line 1)  replaces it with a D-sequent symmetric in $v$  as follows.

Let $x \in \Sup{X}{asym}$ and  $S_0$ and $S_1$ be the D-sequents stating the redundancy of $x$ derived in the left and right branches
respectively. Then \ti{join\_D\_seqs} 
joins $S_0$ and $S_1$ at $v$ producing a new D-sequent $S$. The latter also states the redundancy of  $x$ 
but does not depend on  $v$. D-sequent $S_1$ is replaced in \DS~ with $S$.
If $S_1$ itself does not depend on  $v$, no new D-sequent is produced.  $S_1$ remains in \DS~
as the D-sequent for variable $x$ in \cof{F}{q}.
 
Finally, if the branching variable $v$ is in $X$, \Di derives a  D-sequent stating the redundancy of $v$. Notice that 
$v$ is not currently redundant in \prob{X}{\cof{F}{q}} because \Di does not branch on redundant variables.
 As we mentioned in Subsection~\ref{subsec:br_var_sel}, the variables of $Y = \V{F} \setminus X$ are
assigned in \Di before those of $X$. This means that before $v$ was selected for branching, all free non-detached variables of $Y$ had been
assigned. Besides, every variable  of $X \setminus \Va{q}$ but $v$ has just been proved redundant in \prob{X}{\cof{F}{q}}.
 So, \cof{F}{q} may have only two types of non-redundant clauses: a) clauses having 
only detached variables of $Y$; b) unit clauses depending on $v$.  Moreover, these unit clauses cannot contain literals
of both polarities of $v$ because \ti{merge} is called only when either branch $v=0$ or $v=1$  is satisfied. Therefore, 
$v$ is monotone.
An atomic D-sequent $S$ stating the redundancy of $v$  is built as described in Subsection~\ref{subsec:atomic_d_sequents}
and added to \DS~(line 3). Then \ti{merge} terminates returning \DS.
----------
Let \Di be  called on formula $\Phi=\prob{X}{F}$ with $\pnt{q}=\emptyset$ and $\DS=\emptyset$.
Informally, \Di is correct because a) the atomic D-sequents built by \Di are correct (i.e. they correctly describe
redundancy of quantified variables  in subspaces); b) joining D-sequents 
produces a correct D-sequent; 
c) by the time \Di backtracks to the root of the search tree, for every variable $x \in X$, D-sequent $\emptyset \rightarrow \s{x}$ is derived.
Due to Proposition~\ref{prop:rem_bpts_increm}, this implies that the D-sequent $\emptyset \rightarrow X$ 
holds for the  formula \prob{X}{F}  returned by \Di\!\!.

